Locality Sensitive Hashing for Efficient Similar Polygon Retrieval

Locality Sensitive Hashing (LSH) is an effective method of indexing a set of items to support efficient nearest neighbors queries in high-dimensional spaces. The basic idea of LSH is that similar items should produce hash collisions with higher probability than dissimilar items. We study LSH for (not necessarily convex) polygons, and use it to give efficient data structures for similar shape retrieval. Arkin et al. represent polygons by their "turning function" - a function which follows the angle between the polygon's tangent and the $ x $-axis while traversing the perimeter of the polygon. They define the distance between polygons to be variations of the $ L_p $ (for $p=1,2$) distance between their turning functions. This metric is invariant under translation, rotation and scaling (and the selection of the initial point on the perimeter) and therefore models well the intuitive notion of shape resemblance. We develop and analyze LSH near neighbor data structures for several variations of the $ L_p $ distance for functions (for $p=1,2$). By applying our schemes to the turning functions of a collection of polygons we obtain efficient near neighbor LSH-based structures for polygons. To tune our structures to turning functions of polygons, we prove some new properties of these turning functions that may be of independent interest. As part of our analysis, we address the following problem which is of independent interest. Find the vertical translation of a function $ f $ that is closest in $ L_1 $ distance to a function $ g $. We prove tight bounds on the approximation guarantee obtained by the translation which is equal to the difference between the averages of $ g $ and $ f $.

==> futureIdeas.tex <==
\subsection{Instead of polygons we can work with curves as well}
Also regular curves have their turning function, and if we can assume something about the nature of the curve, e.g., bounded curvature, then having the same curve with the turning function starting with shift $\eps$ compared to the other, their $D_1$ distance can be bounded as a function of $\eps$, so we conclude that quantizing reference points can work for the approximated setting.

\subsection{Generalizing this to 3d polyhedra}

\subsection{Relaxations and simpler settings}
Working with triangles, working with convex shapes (this means the turning function is monotonous. This specifically means that we can do a 2-step alignment process by first reducing the functions' mean, and then doing the same for the y-axis, i.e., flipping the x/y axes, and reducing the mean yet again from each function.)

\subsection{To deal with function shift} We can transform each step function to the set of pairs (step,the pointer to the next step) over all steps (the last step’s next step is the first step).
For example the function $[0,1/3  ]\to 0.2,[1/3,2/3  ] \to 0.4,[2/3,1 ]\to 0.6$ maps to the set:
$\{([0,1/3  ] \to 0.2,[1/3,2/3  ]  ),([1/3,2/3  ] \to 0.4,[2/3,1 ]),([2/3,1 ] \to 0.6,[0,1/3  ])\}$.

\subsection{Work with the $L_2$ distance instead of the $ L_1 $ distance}
We can work with $ D^{al}_{L_2}(f,g)=\sqrt{\int_{0}^{1} \left(f(x)-g(x)\right)^2 dx} $.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{"minimal difference alignment"}
	\caption[]{Minimal Difference Alignment. May be useful for the approximation of the hash for $ D^{add}_{L_2} $.}
	\label{fig:minimal-difference-alignment}
\end{figure}

\subsubsection{A hash for $ D_2^{al} $, but in the wrong direction}
We show a hash for $ D_2^{al} $, which gives a collision with probability exactly the distance. However this is bad, as we want the chance of collision to decrease w.r.t.\ the distance, and not increase w.r.t.\ it.

We define the symmetric hash for data polygons, and the query polygon.
Let $ x,y_1,y_2\sim U([0,1]^3) $, and define the data hash as:
\[h^{Data}_{x,y}(P)=\left(sgn(t_P(x)-y_1),sgn(t_P(x)-y_2)\right),\]
and define the query hash as:
\[h^{Query}_{x,y}(Q)=\left(-sgn(t_Q(x)-y_1),-sgn(t_Q(x)-y_2)\right),\] i.e., flipping the results of the data hash. One can see that $ P(h^{Query}_{x,y}(Q)=h^{Data}_{x,y}(P)) =\left(D_2^{al}(P,Q)\right)^2$.

\subsection{Other possible remedies for the vertical shift distance}
Other ideas that may remedy the additions: 
\begin{enumerate}
	\item Save in the database multiple additions of the function in quantized additions.
	\item Use the symmetric hash $ h_{x_1,x_2,y}(P)=sgn\left(\frac{t_P(x_1)-t_P(x_2)}{2}-y\right) $.
\end{enumerate}

\subsection{Possible remedies for the horizontal (+vertical) shift distance}
In a hash: take a random sequence of points and signes +/-, where for each function we compute the best horizontal shift of the turning function for those points such that the function is above all points with + and below all points with -. (Or alternatively with no +/-, and just maximizing the number of points below the function).
	The hash could be the number of such food points in the vertical shift.
	
	This hash assumes the functions are calibrated vertically, i.e., subtracted the mean...
	
	
Any other hash that makes some randomization, and calculates the optimal vertical shift of the function w.r.t.\ that randomization, and returns some hash as a function of the optimal value, sounds like a good idea...














